FAST-ASKAP Synergy: Quantifying Coexistent Tidal and Ram Pressure Strippings in the NGC 4636 Group

Combining new HI data from a synergetic survey of ASKAP WALLABY and FAST with the ALFALFA data, we study the effect of ram pressure and tidal interactions in the NGC 4636 group. We develop two parameters to quantify and disentangle these two effects on gas stripping in HI-bearing galaxies: the strength of external forces at the optical-disk edge, and the outside-in extents of HI-disk stripping. We find that gas stripping is widespread in this group, affecting 80% of HI-detected non-merging galaxies, and that 41% are experiencing both types of stripping. Among the galaxies experiencing both effects, the two types of strengths are independent, while two HI-stripping extents moderately anticorrelate with each other. Both strengths are correlated with HI-disk shrinkage. The tidal strength is related to a rather uniform reddening of low-mass galaxies ($M_*<10^9\,\text{M}_\odot$) when tidal stripping is the dominating effect. In contrast, ram pressure is not clearly linked to the color-changing patterns of galaxies in the group. Combining these two stripping extents, we estimate the total stripping extent, and put forward an empirical model that can describe the decrease of HI richness as galaxies fall toward the group center. The stripping timescale we derived decreases with distance to the center, from $\mathord{\sim}1\,\text{Gyr}$ beyond $R_{200}$ to $\mathord{\lesssim}10\,\text{Myr}$ near the center. Gas-depletion happens $\mathord{\sim}3\,\text{Gyr}$ since crossing $2R_{200}$ for HI-rich galaxies, but much quicker for HI-poor ones. Our results quantify in a physically motivated way the details and processes of environmental-effects-driven galaxy evolution, and might assist in analyzing hydrodynamic simulations in an observational way.

==> hack.tex <==
%auto-ignore
% hackings
\makeatletter
\AtBeginDocument{
  \newcommand*{\cjkname}[2]{#1 (#2)}
  \@ifpackageloaded{CJK}{}{
    \@ifpackageloaded{xeCJK}{}{
      \renewcommand*{\cjkname}[2]{#1}
    }
  }
}
\usepackage{etoolbox}
% make appendices autoref work
\newcommand*{\@checkappendixparam}[1]{%
  \def\@checkappendixparamtmp{#1}%
  \ifx\Hy@param\@checkappendixparamtmp
    \let\Hy@param\Hy@appendixstring
  \fi
}
\apptocmd{\appendix}{%
  \patchcmd{\hyper@makecurrent}{%
      \edef\Hy@param{#1}%
    }{%
      \edef\Hy@param{#1}%
      \@checkappendixparam{subsection}%
      \@checkappendixparam{subsubsection}%
  }{}{}%
}{}{}
% make footnote alignment right
\patchcmd{\ltx@foottext}{%
  .5\textwidth\advance\hsize-18pt}{%
  \linewidth\advance\hsize-1.8em%
}{}{}
% fix acknowlefgement line numbering
\patchcmd{\acknowledgments}{%
  \begin{internallinenumbers}}{%
  \ifnumlines\begin{internallinenumbers}\fi%
}{}{}
\patchcmd{\endacknowledgments}{%
  \end{internallinenumbers}}{%
  \ifnumlines\end{internallinenumbers}\fi%
}{}{}
% table
\patchcmd{\enddeluxetable}{%
  \null
}{}{}{}
% pagebreak
\renewcommand\ApjSectionpenalty{\@M}
\makeatother

